PropertyDAG: Multi-objective Bayesian optimization of partially ordered, mixed-variable properties for biological sequence design

Bayesian optimization offers a sample-efficient framework for navigating the exploration-exploitation trade-off in the vast design space of biological sequences. Whereas it is possible to optimize the various properties of interest jointly using a multi-objective acquisition function, such as the expected hypervolume improvement (EHVI), this approach does not account for objectives with a hierarchical dependency structure. We consider a common use case where some regions of the Pareto frontier are prioritized over others according to a specified $\textit{partial ordering}$ in the objectives. For instance, when designing antibodies, we would like to maximize the binding affinity to a target antigen only if it can be expressed in live cell culture -- modeling the experimental dependency in which affinity can only be measured for antibodies that can be expressed and thus produced in viable quantities. In general, we may want to confer a partial ordering to the properties such that each property is optimized conditioned on its parent properties satisfying some feasibility condition. To this end, we present PropertyDAG, a framework that operates on top of the traditional multi-objective BO to impose this desired ordering on the objectives, e.g. expression $\rightarrow$ affinity. We demonstrate its performance over multiple simulated active learning iterations on a penicillin production task, toy numerical problem, and a real-world antibody design task.

==> scratch.tex <==
% design space vast, give number for antibody repertoires, computatinoal methods allow intelligent selection inductive biases physics, chemistry
Designing biological sequences entails searching over vast combinatorial design spaces. Recently, deep sequence generation models trained on large datasets of known, functional sequences have shown promise in generating physically and chemically plausible designs \citep[e.g.][]{biswas2021low,das2021accelerated,gligorijevic2021function}. Whereas these models accelerate the design process, limited resources place a cap on how many designs we can characterize \textit{in vitro}. To first order, characterization involves producing the design, confirming its pharmacology, and evaluating whether it is active against a given drug target of interest. If found to be potent, the design is then assayed for \textit{developability} attributes---physicochemical properties that characterize the safety, delivery, and manufacturability \citep{jarasch2015developability}. Only once a design is validated in the wet lab and undergoes multiple rounds of optimization can it proceed down the drug development pipeline to preclinical development and clinical trials, where its performance is tested \textit{in vivo}. 

% Need to choose which ones to characterize. Initial dataset often too small, if at all. 
Because the wet lab cannot provide feedback on all of the candidate designs, we take an iterative, data-driven approach to select the 


%select the most promising subset predicted to carry all the desired properties. We take an iterative, data-driven approach to The decision made in a single shot will be poor based on a fixed initial dataset, which is often too small, if there is one at all. We cast this problem as Bayesian optimization (BayesOpt), a class of black-box optimization  emerges as a  

%The  motivates us to move to an iterative, data-driven search paradigm. In this context, Bayesian optimization emerges as a 


% The high cost of failing any of these criteria at a late stage in drug development has led to considerable efforts at predicting developability on the basis of sequence motifs and experimentally determined biophysical properties (1–15).

% Design generation is cheap and cost increases as proceed down the drug pipeline. Want to select design candidates likely to pass potency and developability screening. Fixed dataset not applicable. Active learning! Bayesian optimization sample-efficient, principled way to navigate the exploration-exploitation tradeoff in the design space

% Often, multiple properties to optimize for. Multi-objective BO. Pareto front. Namely qEHVI, qNEHVI. 


% Developability properties high tailed

% Assumptions: generation (sampling of design candidates) kept separate from inference and selection (can cite Sam's paper for c.f.), not necessary but batched setting (parallel)
%State assumptions. Sampling separate from inference and selection, unlike e.g. lambo. something about asynchronous development of sequence generators and surrogates in practical industry setting

%Often, we benefit from defining an objective as a discrete-valued variable, the measurements for which are obtained by binning the measurements of a continuous-valued variable. For instance, we care about whether a protein expresses \textit{in vivo} in volumes past a threshold yield, but not so much about the precise yield level. Moreover, the experimental scatter in the yield measurements tends to increase as the average yield level increases, so the yield measurements provide carry little signal past the threshold level. 

%Biological properties tend to be zero-inflated -- that is, they are high-tailed and bimodal, where one mode represents ``zero,'' or null, values whereas the other represents (see what zero-inflated paper uses). In this case, we may benefit from course-binning the continuous-valued measurements into binary values and performing classification. Moreover, we often 
%Often, a surrogate model models each objective independently and the models are input to a multi-objective acquisition function, such as the expected hypervolume improvement (EHVI).  We impose a partial ordering of properties such that We present <name>, where  propose a property dag to introduce dependencies between properties in partial ordering.

%Use case considered:(1) the objectives are zero-inflated and/or mixed-variable, i.e. contains both discrete and continuous values, and (2) there is an experimental dependency that motivates a partial ordering of properties.

PropertyDAG sits on top of the existing BayesOpt framework to make it amenable to common scenarios in drug design. It interacts with 



\begin{table}[ht]
  \caption{Predictive performance on joint positives in the test set for the antibody design task}
  \label{tab:ab_metrics}
  \centering
  \begin{tabular}{lll}
    \toprule
    Acquisition     & {}     & {Affinity $\log p^a$} \\
    \midrule
    Random  
    & {} 
    & {$-7.2^{+11.0}_{-11.0}$}     \\
    qNEHVI  
    & {} 
    & {$-5.0^{+7.8}_{-7.8}$}      \\
    qNEHVI-DAG  
    & {}       
    & {$-2.6^{+3.7}_{-3.7}$}  \\
    \bottomrule
  \end{tabular}
\begin{flushleft}
{\footnotesize{$^a$ Log posterior density on binding affinity evaluated at the measurements, averaged over five data splits. Higher is better. Range indicates the upper and lower 1-$\sigma$ across the test set, each averaged over the five data splits.}}\\
\end{flushleft}
%\vspace*{-0.7cm}
\end{table}
\normalsize


\begin{figure}[h!]
\floatbox[{\capbeside\thisfloatsetup{capbesideposition={right, top},capbesidewidth=6cm}}]{figure}[\FBwidth]
{\caption{Number of joint positives in the three objectives over ten simulated active learning iterations for the Penicillin dataset. Error bands are standard deviations over five trials. The qNEHVI-DAG acquisition significantly outperforms qNEHVI and random acquisitions. }\label{fig:penicillin}}
{\includegraphics[width=0.4\textwidth]{figs/penicillin_joint_pos_v3.pdf}}
\end{figure}



